Undermining Mental Proof: How AI Can Make Cooperation Harder by Making Thinking Easier

Large language models and other highly capable AI systems ease the burdens of deciding what to say or do, but this very ease can undermine the effectiveness of our actions in social contexts. We explain this apparent tension by introducing the integrative theoretical concept of "mental proof," which occurs when observable actions are used to certify unobservable mental facts. From hiring to dating, mental proofs enable people to credibly communicate values, intentions, states of knowledge, and other private features of their minds to one another in low-trust environments where honesty cannot be easily enforced. Drawing on results from economics, theoretical biology, and computer science, we describe the core theoretical mechanisms that enable people to effect mental proofs. An analysis of these mechanisms clarifies when and how artificial intelligence can make low-trust cooperation harder despite making thinking easier.

==> removed.tex <==


\newpage

%% equalizing the costs across types eliminates the power of the signal.
%% "big gesture" -- reveals the future expected utility from the relationship
%% Veblen Good? -- 
%% opportunity cost -- proving committment?

%% types have same benefit, but differential cost
%% (college degree example)
%% same costs but different benefits
%% (driving to see gf)

%% relative effort vs absolute
%% when does watermarking work?

% \begin{outline}[enumerate]
%     \0 \noindent \textbf{Introduction: Cognitive Resources, Costly Signalling, and Mental Proof of Work}
%         \1 Generative AI has the potential to greatly reduce the cognitive costs of many activities. In this Perspective, we show that, counterinutitively, this increase of efficiency can have damaging effects on the social fabric, by the vitiation of costly signalling. We distill work from economics, theoretical biology, and cryptography into a key insight: the existence of what we call ``mental proof of work'' enables key mechanisms necessary for human \textbf{cooperation}, \textbf{evaluation}, and \textbf{coordination}. When cognitive costs are driven to zero by Generative AI, however, we should expect that all three domains will be adversely affected. %Our theoretical framework can be applied to pressing questions in policy, law, systems design, and social theory. %\cite{jain2023contextual} on ``Contextual Confidence and Generative AI''
%         \1 First, some definitions. Cognitive costs are those associated with thinking: among other things, the efforts required to pay attention, to focus carefully, to mull over, ponder, revise, and transform beliefs, and to mentally translate one representation into another. These include both the psychological costs required to think (the energy to think, potentially about aversive or unpleasant things) (CITE studies that show people find thinking hard, draining, etc), and the opportunity costs of thinking about one thing instead of another.
%         \1 Our proposal may seem counterintuitive, because a great deal of attention has been devoted to the positive aspects of reducing cognitive costs---by making hard thinking easier, we expect to increase productivity, reduce inefficiency, and increase the rate of scientific discovery and innovation (CITE papers on the economic impact of AI). Attention to the negative aspects has often focused on either the second-order effects (e.g., unemployment CITE) that come only after the benefits have been realized, or on the ways that Generative AI may fail to think well (hallucinations CITE and bias CITE).
%         \1 Longstanding results in the economics of \emph{costly signalling}, however, suggest that there can be significant, and significantly negative, first-order effects to reducing the costs of cognitive effort. It can be socially beneficial to keep the costs of certain behaviors high even when they do not, in themselves, create harms or generate externalities. The seeming paradox arises from the game-theoretic logic of costly signaling; making some benefits more costly than they need to be can have a net-positive outcome.
%         \1 To see this consider the practice of paying someone a compliment. While an (honest) compliment has informational value---it informs me of a positive power or property I possess--it is also, more often than not, a way of building relationships.
%         \1 One way it serves to build relationships is simply that compliments can feel good. However, only the most socially inexpert would see this as the primary mechanism: what matters is the thoughtful compilment, one that demonstrates that one has paid attention to the recipient---a scarce resource which could otherwise be applied to other valuable objectives. Giving such a compliment \emph{proves} (at some degree of confidence) that the sender invested attention, which in turn proves that they value the relationship at at least the cost of the cognitive investment. That investment can involve both perceptive attention (watching the person closely over a period of time), theory of mind (determining what the person most values, and how they perceive the sender), and mental simulation (considering what forms of praise, in what contexts, might be well-received).
%         \1 As in the apology case, the role of mental costs is crucial. The power of the compliment is greatly reduced if the recipient learns, for example, that the sender was given the wording by ChatGPT. If Generative AI can automatically scan a person's social media feed, deduce their emotional weak spot, and provide truthful but empathetic language to re-enforce it, we might become happier---but the social role of compliments in signalling the utility of a relationship, and thus enabling cooperation, might be eliminated. In reducing the cognitive burden, Generative AI might give us more powerful compliments, but weaker relationships.
%         \1 The compliment example shows how costly signalling can provide honest information about a person's utility. It can also provide honest information about a person's knowledge and abilities. To see this, consider a recent experience of the authors (SD), who received an (e-mail) request from a student for an extension on a late assignment. The request appeared to demonstrate that the student understood the burden of late submissions to the TAs and professor, and the role of deadlines in pacing out learning. It did so by proof of mental work: if the student did not understand the situation---if they did not have a good mental model of how deadlines worked in a classroom context---they would have found it far more costly, if not impossible, to describe it so well in an e-mail. Given the larger goals of the course, it would be natural, in turn, for SD to be influenced by such a proof when responding to the inevitable request for an extension: by (apparently) proving that the student understood certain things, the apology appeared to obviate the need for a tedious paternalistic lecture or monitoring that the student would find burdensome.
%         \1 That proof, however, relies upon the existence of cognitive costs. If the e-mail had been written, as SD later suspected, by a Generative AI system such as ChatGPT, the proof would be undermined. 
%         \1 These two examples motivate the basic claim of our Perspective: that an apparent benefit of Generative AI can, in some situations, lead to unexpected inefficiencies. As we will show, these inefficies appear in three distinct domains: cooperation (where utility questions are at stake), evaluation (where ability questions are at stake), and coordination (where both utility and ability come into play).

\begin{outline}[enumerate]
\0 \textbf{Signaling Theory}
    \1 A wide variety of social behaviors rely on the capacity for interacting parties to communicate privately held information to one another. In many contexts, all parties share a common interest in the faithful transmission of accurate information, meaning that senders can honestly express themselves and receivers will interpret what is expressed at face value---a situation game theorists refer to as a ``cheap talk equilibrium'' \cite[see][]{farrell1996cheap}.
    \1 When lying is clearly beneficial, however, merely stating information is no longer credible, and senders must endeavor to \emph{prove} the validity of their claims. (NOTE: Extant work on signaling theory has focused on situations where incentives to lie undermine the credibility of direct expressions of information, but many of the cases we're interested in are also constrained by the difficulty---often, impossibility---of transmitting certain forms of information; e.g., one's mental model of another person.)
    \1 A variety of social mechanisms help facilitate communication in such situations, such as trust and reputation \citep{fehr2009economics}, norms \citep{elster1989social}, and formal institutions \citep{north1991institutions}. However, these remedies are not always available, \emph{e.g.}, at the beginning of a relationship before trust has yet to be established or when the information in question is difficult to objectively verify.
    % such as perjury laws. 
    % (cultivated through repeated interactions, conferred by institutions, \emph{etc.}), social or professional norms, formal punishment, and the law. However,     
    \1 Signaling theory \citep{spence1973job,zahavi1975mate} demonstrates that it is still possible for rational agents to communicate in such situations, specifically by engaging in behaviors that would be self-defeating unless they expected a fact about the world to be true.
    \1 The central insight of the theory is that rational agents only undertake actions that yield expected benefits that outweigh their expected costs. In particular, if the action in question benefits two individuals equally but one undertakes it while another desists, then it must logically be the case that the former expects it to entail lower costs than the latter does. 
    \1 When, further, this decision is made in the presence of an observer who will interpret  behavior in this way, acting gains the additional ``signaling'' benefit that it \emph{distinguishes the acting agent as someone who incurs relatively lower expected costs than their peers}. Even though the action confers these signaling benefits, the high cost of engaging in it naturally prevents those with high costs from exploiting it to their advantage. Hence, the signal cannot be faked and constitutes a credible channel for communicating private information.
    \1 Game theorists describe such an interaction as a``separating equilibirum.''
    \1 The integrity of a signaling equilibrium (and its resulting ability to communicate  information trustlessly) critically depends on not only the presence of costs, but also the differential structure of costs across different subtypes.
    \1 note also that the information communicated must be personal in nature because signaling equilibira can only communicate facts about your personal cost to act.
    % note! we want to emphasize the practical importance of trustlessness in modern communication / society. 


\0 \textbf{Cooperation}

\1 Many forms of cooperation become possible when people realize their intentions are aligned. However, there are sometimes reasons to fake this. Costly signalling makes it possible to provide an honest signal.
\1 Utility signalling -- this is something that enables forms of cooperation that rely on aligned incentives.
\1 Compliment example (already done)
\1 How does this work in the compliment e-mail?
\1 Length is an obvious one; but also there are the two sentence compliments that could not have been produced without a lot of work

\0 \textbf{Evaluation}

\1 Ability signalling.
\1 Kind of like using ChatGPT to cheat.
\1

\0 \textbf{Coordination}

\1 If you know about X, it implies that other people do too, so X is what we coordinate around (culturally, etc)
\1
\1

\0 \textbf{Conclusion}


\newpage

General Categories of Social Mental Proof:







General thoughts:
- Many social proofs are routine / expected and are most notable when they are “conspicuously absent” (e.g., forgetting an anniversary)
- Signaling behaviors can only prove facts about one’s personal costs \& benefits. Someone can use signaling to prove that they themselves are in love or know calculus... but not that someone else is in love or knows calculus.

Credibly transmitting information in cases where you can lie.




Cost examples: the college degree.
Benefit examples: the marriage proposal.

It only works for the \textit{actor's} costs and benefits.

Zero-knowledge examples where you want to keep knowledge secret:
    - Proving you know someone famous but keeping the way in which you met secret (because it's not actually highly impressive)
    - You're a consultant and don't want your client to understand how to replicate you

Human capital is often \textit{only} useful when it can be demonstrated; for example, because you need physical capital (a chemistry lab) to use your human capital (your knowledge of chemistry). Mental proofs play an instrumental role in facilitating the process of matching these two forms of capital. Also applies when you use proofs of existing human capital to become eligible for further human capital investment!


When do we become legible?

We've focused on the cooperative / pro-social cases, but mental proofs can also be used for adversarial purposes.



\newpage


    \0 \textbf{Theoretical Review \& Distillation}
        %
        \1 Overview the theoretical core of costly signaling
            \2 Economics \cite{spence1973job}
            \2 Biology: introduced by \cite{zahavi1975mate};  formalized using game theory by \cite{grafen1990biological}. Applied to explain altruism by \cite{gintis2001costly}
            \2 Core theoretical take-aways \& essential conditions. A non-degenerate correspondence between action and ``type'' (\emph{i.e.} a hidden cognitive state), called a ``separating equilibrium,'' requires:
                \3 Somewhat trivially, at multiple types and multiple behaviors (both can be discrete or continuous). For simplicity, we will focus on the case when there are two types and a single action (which can be either taken or not taken). We usually call one type the ``high'' type and the other type the ``low'' type. For example, high/low commitment, knowledge, \emph{etc.}
                \3 \textbf{Asymmetric information}: The individual contemplating the action's type is not known to external observers. (Whether the acting agent knows, or even thinks about, their type is immaterial.)
                \3 The net benefit (benefit minus cost) for taking the action must be positive for one type and negative for the other. If the net benefit is positive for both, both would take the action, and it would reveal nothing; similarly, if the net benefit is negative for both, neither would take the action, and it would reveal nothing.
                \3 If both types receive positive absolute benefit from being perceived as the high type, then a separating equilibrium necessarily requires that performing the action is    
                \3 Costs do not necessary need to be realized to perform their intended function — they can be potential. For example, a credible promise to take someone's call (and, hence, furnish them with your attention) serves as a social proof of your commitment to the relationship, even if it is never tested.
        \1 \emph{Mental resource costs secure acts of mental proof.}
        
        %
    \0 \textbf{Cooperation, Coordination, \& Cooperation}
        %
        \1 As alluded to above, mental proofs are vital to three broad and consequential classes of social behavior: cooperation, evaluation, and coordination.
        \1 The first, \textbf{cooperation}, refers to situations where individuals use mental proof to communicate their level of commitment, sincerity, or allegiance, both to one another.  
            \2 The prototypical example is an apology letter. If someone sends you a long and heartfelt apology letter that clearly took a great degree of personal reflection, effort, and courage to write, we naturally judge their sincerity as greater than someone who ``merely apologizes,'' especially in a brief and formulaic manner. 
            \2 Sketch out how this example maps onto the core of costly signaling:
                \3 Differential cost of length / effort on letter for the sincere versus insincere
                \3 zero-knowledge proofs: Desire to *demonstrate* that you have performed reflection / remorse / etc. even if you cannot expose these computations to your interlocutor directly.
        \1 The second, \textbf{evaluation}, refers to situations where people use mental proof to reveal \emph{knowledge} or \emph{mental capacity}.
            \2 A prototypical example is the SAT assessing someone's vocabulary. This correlates with time spent reading, which correlates with curiosity, intelligence, and a number of other unobservable qualities. 
            \2 We frequently probe people on situations they could not have foreseen, and therefore memorized (theoretical parallel to zk-proofs). This requires, for example, that tests span broad enough topic domains that people can't predict the questions.
                \3 GenAI undermines this because it can immediately and intelligently recall a huge breadth of knowledge.
        \1 The third, \textbf{coordination}, refers to situations where people use mental proof to reveal that others are focusing on, or committed to, a particular social plan or set of cultural objects.
            \2 If everyone on twitter has hot takes about a particular news story, proves that it's culturally relevant (multiple equilibrium and historical contingency play a huge role, of course).
            \2 Bitcoin's computational proof of work system relies on the correlation between two activities: (1) hashing and (2) tracking the right blockchain. Only the hash can be publicly verified, but it \emph{proves} that whoever submitted it is tracking the right blockchain.
            \2 Analogous proof mechanisms help to establish common knowledge in social settings \cite{chwe2013rational}
        %
    \0 \textbf{Current Issues \& Applications}
        %
        \1 Education
            \2 Verifying that students are ``doing the work'' that is necessary for learning (input monitoring)
            \2 Testing for comprehension, memorization, \emph{etc.} (output monitoring)
        \1 Hiring
        \1 Relationships, dating, \& marriage
        \1 Social \& political discourse?
        \1 A specific policy/technical example: watermarking
            \2 When does watermarking work, when does it not work? Cryptographic keyboards?
        \1 Face-to-face?
        \1 Mental proofs: more important early on in a relationship?
\end{outline}

\newpage
\section{Recent Publications}

\begin{outline}
    \1 \cite{jain2023contextual}
\end{outline}

















\section{Requirements}

The full list of submission requirements can be found \href{https://www.nature.com/nature/for-authors/other-subs}{here}. In brief:

\begin{itemize}
    \item ``The synopsis should outline the basic structure of the article; list the material to be covered with an indication of the proposed depth of coverage; and indicate how the material will be logically arranged.
    \item The synopsis should be accompanied by a 300-500 word outline of the background to the topic which summarizes the progress made to date and should also make the case succinctly for publication in a topical, interdisciplinary journal.
    \item Synopses prepared at this level of detail enable Nature's editors to provide editorial input before they commission the article, and can reduce the need for substantial editorial revisions at a later stage.
    \item The synopsis should include any very recent, key publications in the area.''
\end{itemize}

So, it looks like a ``synopsis'' \emph{and} a 300-500 word outline? The former seems a bit underspecified. On the article format:

\begin{itemize}
    \item ``Perspective articles are intended to provide a forum for authors to discuss models and ideas from a personal viewpoint. They are more forward looking and/or speculative than Reviews and may take a narrower field of view. They may be opinionated but should remain balanced and are intended to stimulate discussion and new experimental approaches.''
    \item ``All Reviews start with a 200-word maximum preface, which should set the stage and end with a summary sentence. 
    \item Reviews vary in length depending on the topic and should not generally be more than 9 pages long... As a guideline, 5000 words, 4 moderate display items (figures/tables/boxes) and a modest citation list (no more than 150 references) will occupy 9 pages.''
\end{itemize}

\newpage
\section{Notes}



        % \1 Hence, apparently self-defeating behaviors often do, in fact, confer benefits because they credibly communicating unobservable facts about an agent's preferences and abilities to others---\emph{e.g.}, one's intelligence to hiring committees (in the former example) and genetic fitness to sexual mates (in the latter).  
